Vertex finding in neutrino-nucleus interaction: A Model Architecture Comparison

We compare different neural network architectures for Machine Learning (ML) algorithms designed to identify the neutrino interaction vertex position in the MINERvA detector. The architectures developed and optimized by hand are compared with the architectures developed in an automated way using the package "Multi-node Evolutionary Neural Networks for Deep Learning" (MENNDL), developed at Oak Ridge National Laboratory (ORNL). The two architectures resulted in a similar performance which suggests that the systematics associated with the optimized network architecture are small. Furthermore, we find that while the domain expert hand-tuned network was the best performer, the differences were negligible and the auto-generated networks performed well. There is always a trade-off between human, and computer resources for network optimization and this work suggests that automated optimization, assuming resources are available, provides a compelling way to save significant expert time.

==> part1.tex <==
\section{Introduction}
 Right now, various neutrino experiments and  other high energy experiments have been using  ML based algorithm rigorously  at reconstruction level to maximize the physics output from the data  as well as at the analysis level. Hence it is very important  to optimize our ML models over its different hyper parameters so that it gives best output. However, optimizing a appropriate set of hyper parameters for different datasets is not only time consuming but also a tedious task. A group of Scientists from  Oak ridge national Laboratory have developed a revolutionary package named "Multi-node Evolutionary Neural Networks for Deep Learning" aka MENNDL which helps to address the model selection problem and ease the demands on data researchers. MENNDL leverages a large number of compute nodes which  communicate over MPI to distribute the task of finding the optimal hyper-parameters across the nodes of a supercomputer. In 2017 ALCC project, ORNL group worked together with MINERvA and NOvA researchers. They used the simulated Neutrino events from MINERvA and generate several models using MENNDL package for vertex finding problem optimizing over different hyper parameters. It is noted that, these models are primarily optimized over short run period (only 5000 iterations) and CAFFE API has been used. 
As mentioned above, MENNDL provided several models for vertex finding problem. Among them, I chose nine different models depending on their validation accuracy (which means how accurately the model predicts the output for validation sample) when they trained over the short run period (5000 iterations). Next, I trained those nine models using anti-neutrino events for long run period and checked the validation accuracy. I selected one of them as "best" model comparing that accuracy number. Next, I consider two artisanal models (Tensorflow and Caffe API based) developed inside MINERvA and trained them using anti-neutirno events. We call them "artisanal" as they were "hand-crafted" and manually optimized by Gabe et.al for neutrino events. It is noted that, the artisanal model, based on tensorflow API, is already being used in the MINERvA collaboration for the vertex finding project in neutrino mode. 
Finally I compared these two artisanal models with the "best" MENNDL-ized model.  For the comparison, I used the same training and testing samples, same batch size. I compared the performance of the models by comparing the accuracy (how accurately model predicts the output) and loss (the error in predicting the output) from different models.
I found that, they have comparable accuracies:
TensorFlow -- 76%
MENNDL-ized -- 74.5%
Caffe Artisanal -- 72.6%
These three models have very different underlying mechanisms, so to keep them at equal footing, I made the same physics studies with these models and compared the plots obtained from them. I found that the results are not much different from one another.  In other words, MENND-ized model behaves similar as the artisanal one.  
So, we found that the model optimized by MENNDL package has similar performance as the artisanal models. Developing the artisanal models needed a rigorous study in order to vary the  different hyper parameters  to be optimized manually and hence consumed a significant human-time as well. On the other hand, MENNDL provides the model which has similar performance as the Artisnal even it is optimized over short-run period. Hence, without any doubt, it can be concluded that MENNDL helps to  save lots of human input and computational time by providing the optimized model which is a promising news for current and future physics community
